Cram\'er-Rao Bounds for Holographic Positioning

Multiple antennas arrays play a key role in wireless networks for communications but also for localization and sensing applications. The use of large antenna arrays at high carrier frequencies (in the mmWave range) pushes towards a propagation regime in which the wavefront is no longer plane but spherical. This allows to infer the position and orientation of a transmitting source from the received signal without the need of using multiple anchor nodes, located in known positions. To understand the fundamental limits of large antenna arrays for localization, this paper combines wave propagation theory with estimation theory, and computes the Cram\'er-Rao Bound (CRB) for the estimation of the source position on the basis of the three Cartesian components of the electric field, observed over a rectangular surface area. The problem is referred to as holographic positioning and is formulated by taking into account the radiation angular pattern of the transmitting source, which is typically ignored in standard signal processing models. We assume that the source is a Hertzian dipole, and address the holographic positioning problem in both cases, that is, with and without a priori knowledge of its orientation. To simplify the analysis and gain further insights, we also consider the case in which the dipole is located on the line perpendicular to the surface center. Numerical and asymptotic results are given to quantify the CRBs, and to quantify the effect of various system parameters on the ultimate estimation accuracy. It turns out that surfaces of practical size may guarantee a centimeter-level accuracy in the mmWave bands.

==> SectionIV.tex <==
 %!TEX root = main.tex
{\color{blue} 
\section{CRB computation  with no \emph{\textsc{a priori}} information about the dipole orientation}
\label{sec:tilted_dipole}


Compared to the ideal case of known dipole orientation, \eqref{eq:crb_ori_x}--\eqref{eq:crb_ori_z} show that no loss is incurred in the estimation of $y_C$ whereas the accuracy in the estimation of $x_C$ and $z_C$ decreases due to the additional non-negative terms $\left|[\mathbf{F}_{ts}]_{31} \right|^2/[\mathbf{F}_{t}]_{33}$ and $\left|[\mathbf{F}_{ts}]_{13} \right|^2/[\mathbf{F}_{t}]_{11}$, respectively.

In Appendix F we show that, in the asymptotic case as $\rho \to \infty$, both $\left|[\mathbf{F}_{ts}]_{31} \right|^2/[\mathbf{F}_{t}]_{33}$ and $\left|[\mathbf{F}_{ts}]_{13} \right|^2/[\mathbf{F}_{t}]_{11}$ go to zero, meaning that, for sufficiently large observation apertures, under Assumption 6 the estimation accuracy does not depend on the exact knowledge of the transmitting antenna orientation.
{\color{BlueGreen} Sarebbe interessante capire se questo vale anche per un dipolo arbitrariamente orientato, sempre ammettendo l'ipotesi di CPL}
}
%\subsection{Asymptotic analysis for CPL when $\rho \to \infty$}
%%\todo[inline]{verify and complete the proof}
%\begin{proposition}
%	For $\rho \rightarrow \infty$ we get
%	
%	\begin{align}\label{Fts31_inf}
%		\dfrac{\left|[\mathbf{F}_{ts}]_{31} \right|^2}{[\mathbf{F}_{t}]_{33}} \rightarrow 0\\\label{Fts13_inf}
%		\dfrac{\left|[\mathbf{F}_{ts}]_{13} \right|^2}{[\mathbf{F}_{t}]_{11}} \rightarrow 0 
%	\end{align}
%	therefore, the asymptotic behaviors of the CRBs are the same as in Assumption~\ref{prop:crb_limits}.
%	
%\end{proposition}
%
%\begin{IEEEproof}
%For $\rho \rightarrow \infty$, $\left|[\mathbf{F}_{ts}]_{13} \right|^2$ is upper limited, as we can state from~\eqref{Fts13}, while the $[\mathbf{F}_{t}]_{11}$ lower bound, \eqref{Ft11}, grows unboundedly with $\log(1+\rho)$. Therefore, the ratio in~\eqref{Fts13_inf} goes to $0$ as $\rho$ grows. Similar considerations also hold for~\eqref{Fts31_inf}, where the denominator $[\mathbf{F}_{t}]_{11}$ lower bound still follows the $\log(1+\rho)$ trend, \eqref{Ft33}, and the numerator is upper bounded for growing $\rho$ (more details in Appendix~\ref{app:calc6D}, section~\ref{ss:fts31_to_inf}).
%%\todo[inline]{per questa ultima frase dovrei aggiungere un minimo di proof, che \'e tranquilla, per\'o sono altre formule da aggiungere e gi\'a non sono poche fin qui... dopo il corso cerco di scriverle in forma compatta}
%
%\end{IEEEproof}
%\begin{figure}
%	\includegraphics[width=\columnwidth]{Figures/Fig_Distance_no-priori.eps}
%	\caption{Fig}
%	\label{fig:us_dist_no-priori}
%\end{figure}





